Mapless Navigation of a Hybrid Aerial Underwater Vehicle with Deep Reinforcement Learning Through Environmental Generalization

Previous works showed that Deep-RL can be applied to perform mapless navigation, including the medium transition of Hybrid Unmanned Aerial Underwater Vehicles (HUAUVs). This paper presents new approaches based on the state-of-the-art actor-critic algorithms to address the navigation and medium transition problems for a HUAUV. We show that a double critic Deep-RL with Recurrent Neural Networks improves the navigation performance of HUAUVs using solely range data and relative localization. Our Deep-RL approaches achieved better navigation and transitioning capabilities with a solid generalization of learning through distinct simulated scenarios, outperforming previous approaches.

==> sections/5_discussion.tex <==
\section{Discussion}
\label{discussion}

% REESCREVER, FALAR QUE TD3 E SAC FICARAM MELHOR QUEDDPG E BUG2. FALAR SEMELHANTE AO QUE FOI FEITO NO PAPER DO JINT 

The evaluation shows an overall increase in performance in navigation through both environments. It is possible to see that our approaches achieve a consistent performance of 100 successful air-to-water navigation trials with also a consistent navigation time ($14.55 \pm 0.87$ and $11.19 \pm 2.86$). In this same scenario, the stochastic performed a little worse in air-to-water navigation but outperformed the deterministic approach in water-to-air navigation. 
In the second scenario, we can see more clearly that a double-critic-based approach with an RNN structure also has a better ability to learn and generalize the environment, including the obstacles and the medium transition. While the state-of-the-art approaches with a MLP structure were not capable of performing the task, our approaches presented once again a consistent performance, especially in air-to-water navigation. Our approaches showed an excellent ability to learn the tasks and the environmental difficulties, not only the scenario itself. That was further addressed in our additional evaluation with agents trained in the first environment only, both first and second environments and the second environment only. Overall, we can conclude that double critic approaches with recurrent neural networks present a consistent ability to learn through scenarios and environments and to generalize between them. Also, our approaches outperformed the BBA algorithm 
% \cbox{BUG2 algorithm - CHamaria de behavior-based algorithm ou algo assim} 
in the rate of successful trials and average time in almost all situations.

It is important to mention that these approaches are extensively evaluated in a realistic simulation, including control issues and disturbances such as wind. Thus, the results indicate that our approach may achieve real-world application if the correct data from the sensing and the relative localization are correctly ensured. Finally, it is also possible to analyze that these new RNN-based approaches provided a more consistent average course of action throughout the environments.
% We can see in Fig.~\ref{fig:cmd} a decrease in the action's standard deviation when compared with the action's standard deviation of the state-of-the-art~\cite{bedin2021deep}. 

% The extensive validation of our proposed reveals a proper behavior for both agents in both environments. The agents were able to learn environmental difficulties, realize the medium transition, and generalize enough to perform the mapless navigation through air and water. Besides that, our agents also learned to bypass obstacles to arrive at a target and managed to outperform a traditional algorithm. We have validated two powerful approaches, which managed to understand the complex behaviors in realistic simulation and that can be used in the real world if guarantying range findings and relative localization data. 

% Specifically, we can also observe that our deterministic approach performed considerably better than our 3DNDRL-S approach in the first and simpler scenario with just simulated wind and a water tank. However, in the second scenario with simulated drilling risers, we can observe based on the results of Table \ref{table:mean_std} and Figs. \ref{fig:traj_nav_1} and \ref{fig:traj_nav_2} that the better exploration policy of the 3DNDRL-S approach made it have a similar or even better performance than our deterministic algorithm. Finally, it is interesting to notice that, besides the fact that our two approaches have fundamental differences in its implementation, the actions generated by each of them at each step of testing when averaged 100 times are quite similar, manly in the second and more complex scenario. We can observe this robustness and consistency in Fig. \ref{fig:cmd}.


